E-TEST prototype design report

E-TEST (Einstein Telescope Euregio-Meuse-Rhin Site and Technology) is a project recently funded by the European program Ineterreg Euregio Meuse-Rhine. This program is dedicated to innovative cross boarder activities between Belgium, The Netherlands and Germany. With a total budget of15MC and a consortium of 11 partners from the three countries, the objective of the project is twofold. Firstly, to develop an eco-friendly and non-invasive imaging of the geological conditions as well as the development of an observatory of the underground in the EMR region. Secondly, to develop technologies necessary for 3rd generation gravitational wave detectors. In particular, it is proposed to develop a prototype of large suspended cryogenic silicon mirror, isolated from seismic vibrations at low frequency. The total budget of the project is equally spread over the two activities. The first activity is not discussed at all in this report. The E-TEST prototype will have some key unique features: a silicon mirror of 100 kg, a radiative cooling strategy (non contact), a low-frequency hybrid isolation stage, cryogenic sensors and electronics, a laser and optics at 2 microns, a low thermal noise coating.

==> ETEST_subsystems/orga.tex <==
\chapterimage{Figures/white.png} 
\chapter{Organisational Overview of ETpathfinder}
\label{sec:orga}

\begin{figure}[htbp!]
\centering
\includegraphics[width=17.5cm]{Figures/ETpathfinder_ornigram_v2.pdf}
\label{fig:wp4_gantt}
\end{figure}

==> ET_Macros.tex <==
\usepackage{framed} 
\usepackage{ifthen}

%%%%%%%%% begin: macros for creating  ET boxes %%%%%%%% 
\newcommand{\titlecolor}{white}
\newcommand{\captioncolor}{white}
\newcommand{\contentcolor}{white}
\newcommand{\ccolor}{\definecolor{citecolor}{rgb}{0,.5,0}}
\newcommand{\lcolor}{\definecolor{linkcolor}{rgb}{.8,0,0}}
\newcommand{\ucolor}{\definecolor{urlcolor}{rgb}{0,0,.7}}
\newcommand{\etboxwidth}{0.975\textwidth}
\newcommand{\etboxskip}{0.0125\textwidth} % this is (1-\etboxwidth)/2
\newcommand{\etboxmargin}{0.5cm}

\floatstyle{ruled} 
\newfloat{ETbox}{t}{lop}[section] %bhp

\newenvironment{ETboxenvironment}[1][\hsize]{%
\def\FrameCommand{\fcolorbox{framecolor}{shadecolor}}%
\MakeFramed{\hsize#1\advance\hsize-\width\FrameRestore}}%
{\endMakeFramed}


%%% The long ET box %%%%
\def\longetbox#1#2#3#4{ 
\definecolor{framecolor}{cmyk}{1,1,1,1}%
\ifthenelse{\equal{#1}{r}}{%
\definecolor{darkred}{rgb}{0.6,0,0}
\definecolor{semidarkred}{rgb}{0.8,0,0}
\floatname{ETbox}{\color{darkred}\large Box}% 
\renewcommand{\titlecolor}{darkred}%
\renewcommand{\captioncolor}{darkred}%
\renewcommand{\contentcolor}{semidarkred}%
\renewcommand{\ccolor}{\definecolor{citecolor}{rgb}{0,0,0.8}}%
\renewcommand{\lcolor}{\definecolor{linkcolor}{rgb}{.0,.8,0}}%
\renewcommand{\ucolor}{\definecolor{urlcolor}{rgb}{0,0.8,0.8}}%
\definecolor{shadecolor}{rgb}{1,0.9,0.7}}{%
\ifthenelse{\equal{#1}{i}}{%
\floatname{ETbox}{\color{blue}\large Box}% 
\renewcommand{\titlecolor}{blue}%
\renewcommand{\captioncolor}{blue}%
\renewcommand{\contentcolor}{blue}%
\renewcommand{\ccolor}{\definecolor{citecolor}{rgb}{0,.5,0}}
\renewcommand{\lcolor}{\definecolor{linkcolor}{rgb}{.8,0,0}}
\renewcommand{\ucolor}{\definecolor{urlcolor}{rgb}{0.9,0.,0.9}}
\definecolor{shadecolor}{cmyk}{.07,.01,0,0}}{%
\ifthenelse{\equal{#1}{h}}{%
\floatname{ETbox}{\color{blue}\large Box}% %%%%%%%%%%%%%%%%%%
\renewcommand{\titlecolor}{blue}%
\renewcommand{\captioncolor}{blue}%
\renewcommand{\contentcolor}{black}%
\renewcommand{\ccolor}{\definecolor{citecolor}{rgb}{0,.5,0}}%
\renewcommand{\lcolor}{\definecolor{linkcolor}{rgb}{.8,0,0}}%
\renewcommand{\ucolor}{\definecolor{urlcolor}{rgb}{0,0,.7}}%
\definecolor{shadecolor}{cmyk}{0,0,.3,0}}{}{}}}%
\vspace{\parskip} 
\color{\contentcolor}
\fboxrule 0.75pt
\setlength{\fboxsep}{\etboxmargin}
\begin{ETboxenvironment}[\etboxwidth] 
\arrayrulecolor{\contentcolor}
\ccolor
\lcolor
\ucolor
\captionsetup{labelfont={color=\contentcolor,bf}, textfont={color=\contentcolor}, labelsep=colon}%, margin=\etboxskip}%
\captionof{ETbox}[#3]{\textcolor{\captioncolor}{\large\bf#3}} 
\captionsetup{labelfont={color=\contentcolor,bf}, textfont={color=\contentcolor},labelsep=colon}%, margin=\etboxskip}  % add something of geometry
#4
\label{#2} 
\end{ETboxenvironment} 
\arrayrulecolor{black} 
\color{black} 
%\definecolor{citecolor}{rgb}{0,.5,0}
%\definecolor{linkcolor}{rgb}{.8,0,0}
%\definecolor{urlcolor}{rgb}{0,0,.7}

}
%%%%%%%%%%  %%%%%%%%


%%%%%%% the one-page ETbox %%%%%%%% 

\def\etbox#1#2#3#4{ 
\definecolor{framecolor}{cmyk}{1,1,1,1}%
\ifthenelse{\equal{#1}{r}}{%
\definecolor{darkred}{rgb}{0.6,0,0}
\definecolor{semidarkred}{rgb}{0.8,0,0}
\floatname{ETbox}{\color{darkred}\large Box}% 
\renewcommand{\titlecolor}{darkred}%
\renewcommand{\captioncolor}{darkred}%
\renewcommand{\contentcolor}{semidarkred}%
\renewcommand{\ccolor}{\definecolor{citecolor}{rgb}{0,0,0.8}}%
\renewcommand{\lcolor}{\definecolor{linkcolor}{rgb}{.0,.8,0}}%
\renewcommand{\ucolor}{\definecolor{urlcolor}{rgb}{0,0.8,0.8}}%
%\floatname{ETbox}{\color{white}\large Box}% 
%\renewcommand{\titlecolor}{white}%
%\renewcommand{\captioncolor}{white}%
%\renewcommand{\contentcolor}{white}%
%\renewcommand{\ccolor}{\definecolor{citecolor}{rgb}{.4,.9,.9}}%
%\renewcommand{\lcolor}{\definecolor{linkcolor}{rgb}{.9,.9,0}}%
%\renewcommand{\ucolor}{\definecolor{urlcolor}{rgb}{0,0.9,.5}}%
%\definecolor{shadecolor}{cmyk}{.0,.8,.7,0}}{%
\definecolor{shadecolor}{rgb}{1,0.9,0.7}}{%
%\definecolor{shadecolor}{rgb}{0.65,0.09,0.09}}{%
\ifthenelse{\equal{#1}{i}}{%
\floatname{ETbox}{\color{blue}\large Box}% 
\renewcommand{\titlecolor}{blue}%
\renewcommand{\captioncolor}{blue}%
\renewcommand{\contentcolor}{blue}%
\renewcommand{\ccolor}{\definecolor{citecolor}{rgb}{0,.5,0}}
\renewcommand{\lcolor}{\definecolor{linkcolor}{rgb}{.8,0,0}}
\renewcommand{\ucolor}{\definecolor{urlcolor}{rgb}{0.9,0.,0.9}}
\definecolor{shadecolor}{cmyk}{.07,.01,0,0}}{%
\ifthenelse{\equal{#1}{h}}{%
\floatname{ETbox}{\color{blue}\large Box}% 
\renewcommand{\titlecolor}{blue}%
\renewcommand{\captioncolor}{blue}%
\renewcommand{\contentcolor}{black}%
\renewcommand{\ccolor}{\definecolor{citecolor}{rgb}{0,.5,0}}%
\renewcommand{\lcolor}{\definecolor{linkcolor}{rgb}{.8,0,0}}%
\renewcommand{\ucolor}{\definecolor{urlcolor}{rgb}{0,0,.7}}%
\definecolor{shadecolor}{cmyk}{0,0,.3,0}}{}{}}}%
\begingroup
\begin{center}   
\begin{minipage}[t]{\etboxwidth} 
\leftskip=\etboxskip
\rightskip=\etboxskip
\definecolor{framecolor}{cmyk}{1,1,1,1}
\begin{framed} 
\vspace{-9pt} 
\arrayrulecolor{\contentcolor}
\begin{shaded}       
\lcolor
\ccolor
\ucolor
\captionsetup{labelfont={color=\captioncolor,bf}, textfont={color=\captioncolor}, labelsep=colon, margin=\etboxskip}%
\captionof{ETbox}[#3]{\textcolor{\captioncolor}{\large\bf#3}} 
\captionsetup{labelfont={color=\titlecolor,bf}, textfont={color=\contentcolor},labelsep=colon, margin=\etboxskip}%\etboxmargin} 
\textcolor{\contentcolor}{#4} 
\label{#2} 
\end{shaded} 
\vspace{-9pt} 
\end{framed} 
\end{minipage} 
\end{center} 
\endgroup
\vspace{9pt} 
\arrayrulecolor{black} 
\color{black} 
%\definecolor{citecolor}{rgb}{0,.5,0}
%\definecolor{linkcolor}{rgb}{.8,0,0}
%\definecolor{urlcolor}{rgb}{0,0,.7}
}
%%%%%%%%%%% end: macros for creating a box %%%%%%%%
%





%%% begin:  macros for creating the Glossary %%%%%%%
\usepackage{ifthen}
\usepackage[cfg, intoc]{nomencl}
\renewcommand{\nomgroup}[1]{%
 \ifthenelse{\equal{#1}{S}}{\vspace{30pt}\item[]\hspace*{-\leftmargin}%
 \rule[2pt]{0.45\linewidth}{1pt}%
 \hfill \textbf{Symbols} \hfill
 \rule[2pt]{0.45\linewidth}{1pt}\vspace{-5pt} \item[]\hspace*{-\leftmargin}\vspace{5pt}\hspace{1.1cm}Please note that some symbols might stand for more than one quantity depending on the context}{%
\ifthenelse{\equal{#1}{A}}{\item[]\hspace*{-\leftmargin}
\rule[2pt]{0.45\linewidth}{1pt}%
\hfill \textbf{Abbreviations} \hfill
\rule[2pt]{0.45\linewidth}{1pt}}{%
\ifthenelse{\equal{#1}{G}}{\vspace{30pt}\item[]\hspace*{-\leftmargin}
\rule[2pt]{0.45\linewidth}{1pt}%
\hfill \textbf{Glossary} \hfill
\rule[2pt]{0.45\linewidth}{1pt}}{}{}}}}
\renewcommand{\nomname}{Nomenclature}
\makenomenclature
       %%% end:  macros for creating the  Glossary %%%%%%%



==> Summary/Summary.tex <==
\chapterimage{Figures/money2.jpg} % Chapter heading image
%Einstein Telescope artists impression copyright Nikhef
%\section{Introduction}
\chapter{Budget Summary}
\label{chap:BudgetSummary}

The overall equipment budget of the ETpathfinder phase 1a/b project is composed of the individual budgets of work packages WP3 to WP7 as follows. We additionally list a budget contingency of 10\%, which is foreseen to cover unexpected expenses, especially for items that have to go through a tendering process and thus precise costings cannot be given in advance.

\begin{table}[htbp]
\centering
    \begin{tabular}{lSS}
    \toprule
    Work Package & {Budget in €, incl VAT} & {Budget in €, excl VAT}\\
    \midrule
    WP3: Cleanroom & 3250000 & 2685950 \\
    WP4: Vacuum System & 4481840 & 3704000 \\
    WP5: Seismic Isolation & 1300000 & 1074380 \\
    WP6: Optics & 3408320 & 2816793 \\
    WP7: Controls & 2321108 & 1918271 \\
    \midrule
    Subtotal & 14761268 & 12199395 \\
    Contingency 10\% & 1476127 & 1219940 \\
    Total & 16237394 & 13419335 \\
    \bottomrule
    \end{tabular}
\end{table}

\begin{figure}
    \centering
        %\label{fig:budget_breakdown}
    \includegraphics[width=0.95\linewidth]{Figures/budget.pdf}
\end{figure}

%Figure~\ref{fig:budget_breakdown} gives a grapahical breakdown of the budget split between the different workpackages.


The subtotal without contingency (14.76\,MEuro) matches pretty well the earlier cost estimates of the proposal (14.50\,MEuro) and we assume the deviation of less than 2\,\% is well within the noise of the accuracy of our knowledge of the costs and hence no cause for major concern. 
However, the Interreg grant did not consider any contingency. If an contingency is found to be necessary, additional funds have to be found. 




==> defs.tex <==
\def\newacronym#1#2#3{\gdef#1{#3 (#2)\gdef#1{#2}}}

%%%%%%%% common commands
\def\gw#1{gravitational-wave#1 (GW#1)\gdef\gw{GW}}
\def\grb#1{gamma ray burst#1 (GRB#1)\gdef\grb{GRB}}

\newacronym{\NR}{NR}{Numerical Relativity}
\newacronym{\GR}{GR}{General Relativity}


\def\th{\textrm{\mbox{\tiny{th}}}}
\def\Tobs{T_{\textrm{\mbox{\tiny{obs}}}}}
\def\Tcoh{T_{\textrm{\mbox{\tiny{coh}}}}}
\def\nd{{\mathbf{n}}_d}
\def\SSB{\textrm{\mbox{\tiny{ssb}}}}
\def\ns{\textrm{\mbox{\tiny{NS}}}}
\def\min{\textrm{\mbox{\tiny{min}}}}
\def\max{\textrm{\mbox{\tiny{max}}}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\N{\textit{\mbox{\tiny{N}}}}
\def \calf {\cal F}
\def\etal{{\it et al.}}

\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\un}[1]{\mathrm{\,#1}}
\newcommand{\ee}[1]{\!\times\!10^{#1}}
\newcommand{\Qhat}{{\widehat{Q}}}
\newcommand{\What}{{\widehat{W}}}
\newcommand{\rd}{\,{\rm d}}
\newcommand{\avec}{\mbox{\boldmath$a$}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\mtot}{\mathrm{M}_{\mathrm{T}}}
\newcommand{\msun}{\mathrm{M}_{\odot}}
\newcommand{\Msun}{\mathrm{M}_{\odot}}
\newcommand{\Mtot}{\mathrm{M}_{T}}

\newcommand{\np}{\vspace{0.2cm}\noindent}


\def\th{\textrm{\mbox{\tiny{th}}}}
\def\Tobs{T_{\textrm{\mbox{\tiny{obs}}}}}
\def\Tcoh{T_{\textrm{\mbox{\tiny{coh}}}}}
\def\nd{{\mathbf{n}}_d}
\def\SSB{\textrm{\mbox{\tiny{ssb}}}}
\def\ns{\textrm{\mbox{\tiny{NS}}}}
\def\min{\textrm{\mbox{\tiny{min}}}}
\def\max{\textrm{\mbox{\tiny{max}}}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\N{\textit{\mbox{\tiny{N}}}}
\def \calf {\cal F}
\def\ie{{\it i.e.}}
\def\eg{{\it e.g.}}
\def\vs{{\it vs.}}
\def\fstat{$\calf$-statistic}
\newcommand{\G}{\mathcal{G}}

% ---- Burst-specific commands.
\newcommand{\cwb}{\textsc{cwb2g}}
\newcommand{\stamp}{\textsc{stamp}}
\newcommand{\stampas}{\textsc{stamp-as}}
\newcommand{\ep}{\textsc{excesspower}}
\newcommand{\xp}{\textsc{x-pipeline}}
\newcommand{\lib}{\textsc{lib}}
\newcommand{\bw}{\textsc{bayeswave}}
\newcommand{\kw}{\textsc{kleine-welle}}
\newcommand{\om}{\textsc{omicron}}  
\newcommand{\bwg}{Burst Group}

% CBC group definitions
\newcommand{\MBTA}{\textsc{\ac{MBTA}}\xspace}
\newcommand{\LLOID}{\ac{LLOID}\xspace}
\newcommand{\GSTLALCBC}{\textsc{Gstlal-CBC}\xspace}
\newcommand{\ahope}{\textsc{aHope}\xspace}
\newcommand{\bayestar}{\textsc{Bayestar}\xspace}
\newcommand{\lalinference}{\textsc{LALInference}\xspace}
\newcommand{\pycbc}{\textsc{pyCBC}\xspace}
\acrodef{CBC}{Compact Binary Coalescence}
\acrodef{GW}{gravitational-wave}
\acrodef{BNS}{binary neutron star}
\acrodef{NS}{neutron star}
\acrodef{NSBH}{neutron star black hole binary}
\newacronym{\BBH}{BBH}{black hole binary}
\acrodef{EM}{electromagnetic}
\acrodef{EOS}{equation of state}
\acrodef{GRB}{gamma-ray burst}
\acrodef{LLOID}{Low-Latency Online Inspiral Detector}
\acrodef{MBTA}{Multi-Band Template Analysis}

% Computing definitions
\newcommand\ligocomputing{LIGO Computing}
\newcommand\tieronesites{Tier-1-Observatories}
\newcommand\tieronecit{Tier-1-Caltech}
\newcommand\tiertwoshared{Tier-2-Shared}
\newcommand\tiertwoother{Tier-2-Other}
\newcommand\ldg{LDG}
\acrodef{LSC}{LIGO Scientific Collaboration}
\acrodef{LDR}{LIGO Data Replicator}
\acrodef{LDG}{LIGO Data Grid}
\acrodef{iLIGO}{initial LIGO}
\acrodef{aLIGO}{advanced LIGO}
\newacronym{\aligo}{aLIGO}{Advanced LIGO}


% from the Observing Scenario Document
\def\aLIGOEarly{60}
\def\aLIGOEarlyU{40 -- 80}
\def\aLIGOMid{100}
\def\aLIGOMidU{80 -- 120}
\def\aLIGOLate{140}
\def\aLIGOLateU{120 -- 170}
\def\aLIGOFinal{200}
\def\aLIGOFinalBNS{215}
\def\AdVInitial{20}
\def\AdVEarly{40}
\def\AdVEarlyU{20 -- 60}
\def\AdVMid{70}
\def\AdVMidU{60 -- 85}
\def\AdVLate{100}
\def\AdVLateU{65 -- 115}
\def\AdVFinal{130}
\def\AdVFinalBNS{145}

% journals
\providecommand{\jcap}[0]{JCAP}
\def\aj{Astronomical Journal}                 % Astronomical Journal
\def\apj{Astrophysical Journal}                % Astrophysical Journal
\def\apjl{Astrophysical Journal Letters}             % Astrophysical Journal, Letters
\def\pasj{PASJ}
\def\apjs{ApJS}              % Astrophysical Journal, Supplement
\def\mnras{MNRAS}            % Monthly Notices of the RAS
\def\prd{Physical Review D}       % Physical Review D
\def\prx{Physical Review X}       % Physical Review X
\def\prl{Physical Review Letters}    % Physical Review Letters
\def\cqg{Classical \& Quantum Gravity}%Classical and Quantum Gravity
\def\nat{Nature}              % Nature
\def\physrep{Physics Reports} % Physics Reports
\def\na{New Astronomy}		% New Astronomy
\def\aapr{Astronomy \& Astrophysics Reviews}	%Astronomy and Astrophysics Reviews
\def\araa{Annual Reviews of Astronomy \& Astrophysics} 
\def\aap{Astronomy \& Astrophysics}

% other
\newacronym{\APPEC}{APPEC}{Astro-Particle Physics European Consortium}
\newacronym{\ILC}{ILC}{International Linear Collider}
\newacronym{\FALC}{FALC}{Funding Agencies for Large Colliders}
\newacronym{\ICFA}{ICFA}{International Committee for Future Accelerators}
\newacronym{\TMT}{TMT}{Thirty Meter Telescope}

